Locally computing edge orientations

We consider the question of orienting the edges in a graph $G$ such that every vertex has bounded out-degree. For graphs of arboricity $\alpha$, there is an orientation in which every vertex has out-degree at most $\alpha$ and, moreover, the best possible maximum out-degree of an orientation is at least $\alpha - 1$. We are thus interested in algorithms that can achieve a maximum out-degree of close to $\alpha$. A widely studied approach for this problem in the distributed algorithms setting is a ``peeling algorithm'' that provides an orientation with maximum out-degree $\alpha(2+\epsilon)$ in a logarithmic number of iterations. We consider this problem in the local computation algorithm (LCA) model, which quickly answers queries of the form ``What is the orientation of edge $(u,v)$?'' by probing the input graph. When the peeling algorithm is executed in the LCA setting by applying standard techniques, e.g., the Parnas-Ron paradigm, it requires $\Omega(n)$ probes per query on an $n$-vertex graph. In the case where $G$ has unbounded degree, we show that any LCA that orients its edges to yield maximum out-degree $r$ must use $\Omega(\sqrt n/r)$ probes to $G$ per query in the worst case, even if $G$ is known to be a forest (that is, $\alpha=1$). We also show several algorithms with sublinear probe complexity when $G$ has unbounded degree. When $G$ is a tree such that the maximum degree $\Delta$ of $G$ is bounded, we demonstrate an algorithm that uses $\Delta n^{1-\log_\Delta r + o(1)}$ probes to $G$ per query. To obtain this result, we develop an edge-coloring approach that ultimately yields a graph-shattering-like result. We also use this shattering-like approach to demonstrate an LCA which $4$-colors any tree using sublinear probes per query.

==> 100-introduction.tex <==
\section{Introduction}
Orienting graph edges while obeying certain constraints has applications in many computational settings. 
For instance, low-out-degree orientation has been studied in the dynamic~\cite{brodal1999dynamic,he2014orienting,berglin2020simple,solomon2020improved,christiansen2022dynamic}, distributed~\cite{ghaffari2017distributed,fischer2017deterministic,ghaffari2018derandomizing,harris2019distributed,su2020distributed,harris2021locality}, and massively parallel computation~\cite{ghaffari2019improved,biswas2022massively} settings.
The general problem of graph orientation is of significant interest as it serves as an important algorithmic tool for other computational problems.
In their celebrated result, when the input is given as a rooted tree where each edge is oriented toward its parent, Cole and Vishkin~\cite{cole1986deterministic} show how to $3$-color a tree in only $O(\log^* n)$ many distributed rounds.
The algorithm of \cite{solomon2020improved} employs low-out-degree graph orientation to obtain a dynamic algorithm for graph coloring, and the works \cite{neiman2015matching,he2014orienting,bernstein2016faster} apply results from dynamic edge orientation in designing algorithms for matching.
To dynamically maintain spanners, the work of \cite{bodwin2016fully} develops a method that also relies on graph orientation. The authors of \cite{even2014deterministic} design a local computation algorithm (LCA) for bounded-reachability orientations (a different class of orientations) to develop an efficient LCA for coloring. 
It is well-known that the low-out-degree orientation and densest subgraph are problems that are dual to each other~\cite{charikar2000greedy,bahmani2014efficient}.
Moreover, graph orientation has applications in small subgraph counting and listing~\cite{bera2019linear,biswas2022massively}.
Our work focuses on low-out-degree orientation in the context of LCAs.

\subsection{The problem of \texorpdfstring{$r$}{r}-orientation}

Given a graph $G$ with $n$ vertices, we consider the problem of orienting its edges such that every vertex has out-degree at most $r$, for some parameter $r$. 
We call such an orientation an \textit{$r$-orientation}.
Letting $\alpha$ denote the arboricity and $\rho$ the pseudo-arboricity of $G$, the best possible achievable value of $r$ is $r=\rho$, and it is also known that $\rho \le \alpha \le \rho + 1$~\cite{picard1982network,westermann1988efficient,blumenstock2020constructive}. 
However, we are also interested in approximation algorithms where we can achieve some value $r \ge \rho$. Since $\rho$ and $\alpha$ differ by at most one, we will mostly compare $r$ to $\alpha$ instead of $\rho$ since it will make some of our algorithms easier to describe.

A line of work~\cite{ghaffari2017distributed,fischer2017deterministic,ghaffari2018derandomizing,su2020distributed,harris2019distributed,harris2021locality} studied this problem in the distributed LOCAL model in which, under different conditions on $\eps \alpha$, they demonstrate algorithms that use $O(\poly \log n)$ rounds to achieve a value of $r=\alpha(1+\eps)$. In particular, Su and Vu~\cite{su2020distributed} provide such an orientation in $\tilde{O}(\log^2 n / \eps^2)$ rounds, while Harris, Su, and Vu~\cite{harris2021locality} improve the dependence on $1/\eps$ from quadratic to linear at the expense of an additional $\log n$ factor in the round complexity.

We consider this problem in the local computation algorithm (LCA) model (fully defined in \cref{sec:lca}), in which the algorithm must be able to orient any input edge such that many copies of the algorithm will, with no interaction between them except for a shared random string, produce a consistent orientation.
To the best of our knowledge, the low-out-degree orientation problem has not been previously studied
in the LCA setting.

A common method for obtaining LCAs from distributed algorithms is the Parnas-Ron paradigm \cite{parnas2007approximating}. 
As we will discuss further in \cref{sec:related}, in the regime we consider, the Parnas-Ron paradigm does not give any nontrivial sublinear-time algorithm.

\subsection{Our results}

As our first result, we show that an LCA that finds an $r$-orientation (even when $r$ depends on $n$) requires at least $\Omega(n^{1/2}/r)$ probes per query, even if the algorithm is randomized and the input graph is a forest (with $\alpha=1$).
\begin{theorem}[Rephrasing of \cref{prop:lower-bound}] \label{thm:lower-bound-arb}
    For any parameter $r$, any LCA randomized algorithm that yields an $r$-orientation with probability at least 0.9 must use at least $\Omega(n^{1/2}/r)$ probes per query in the worst case.
\end{theorem}
In fact, this lower bound holds against an LCA model with relatively strong queries: we allow algorithms to make adjacency-list, adjacency-matrix, and degree probes.

We then show upper bounds for the problem of $r$-orientation in arboricity-$\alpha$ graphs of unbounded degree, with different algorithms for different regimes of $r$. These upper bounds are also polynomial in $n$, though there is some separation between them and the lower bound of $\Omega(n^{1/2}/r)$.

\begin{theorem}[Rephrasing of \cref{prop:ub-1,prop:ub-2,prop:ub-3}]
\label{thm:upper-bound-arb}
    Suppose there is a parameter $r$, and an input graph $G$ of arboricity $\alpha$. Then, if $r \ge 10(\alpha^2 n)^{1/3}$, there is a randomized LCA that can $r$-orient $G$ with at most $\Ot(\max\{\alpha n/r^2, 1\})$ probes per query. Moreover, if $\alpha=1$ (i.e., $G$ is a forest), then there is also an LCA which can do so for any $r$, with at most $\Ot(n/r)$ probes per query.
\end{theorem}
For example, in the case of a forest ($\alpha=1$) and when $r=10n^{1/3}$, this result gives an LCA for $r$-orientation with probe complexity $\Ot(n^{1/3})$. In contrast, the lower bound given by \cref{thm:lower-bound-arb} is $\Omega(n^{1/6})$.

Finally, we consider the bounded-degree case, where $G$ has maximum degree $\D$, in the specific case where $\alpha=1$ (that is, $G$ is a forest). In this case, any orientation achieves $r \le \D$, so the meaningful case to consider is where $r < \D$. We show a sublinear algorithm in the case where $r = \D^{1-\Omega(1)}$:

\begin{theorem}[Rephrasing of \cref{thm:ub-bdd}] \label{thm:ub-bdd-reph}
    Let $r$ be a parameter and $G$ be an input forest with maximum degree $\D$. Then, there is a randomized LCA that $r$-orients $G$, with at most $\D n^{1-\log_\D r + o(1)}$ probes per query.
\end{theorem}

To prove this theorem, we use a concentration bound on the size of connected components of a random subgraph of a bounded-degree forest.
We also use this to derive an LCA for 4-coloring any tree (or forest) with bounded degree in sublinear time.
Specifically, we show the following:

\begin{theorem}%[Special case of \cref{thm:color}]
    Let $G$ be an input forest with maximum degree $\D$, where $\D$ is a constant. Then, there is a randomized LCA that 4-colors $G$ with query complexity $O(n^{1-\beta})$, where $\beta > 0$ is a constant depending on $\D$.
\end{theorem}

\subsubsection{Future directions:}
It remains open whether similar upper bounds for $r$-orientation can be obtained for other families of graphs. We are optimistic that ideas akin to those we develop for \cref{thm:ub-bdd-reph} might yield new upper bounds for minor-free graphs.
This is because minor-free graphs do not expand, which intuitively is required for the coloring approach we design to prove \cref{thm:ub-bdd-reph}.
We also believe that useful tools in tackling this question include LCAs for minor-free partitioning oracles~\cite{hassidim2009local,levi2015quasi,kumar2021random}.
It would be quite interesting to obtain upper bounds for bounded arboricity graphs that go beyond our result \cref{thm:upper-bound-arb} or to bring the lower bound of \cref{thm:lower-bound-arb} up to match the result of \cref{thm:upper-bound-arb} in the case of a forest. 
We expect that techniques we develop to prove \cref{thm:ub-bdd-reph} do not transfer to bounded arboricity graphs, as there are even expanders with arboricity $3$.


\subsection{Related work} \label{sec:related}
% \cite{brandt2016lower}: provide a lower-bound for distributed LLL. They give $\Omega(\log \log n)$ round complexity. They study sinkless orientation.

% \cite{hefetz2016polynomial}: a lower-bound for graph coloring.

% \cite{balliu2022distributed}: give a lower-bound for ruling-sets in LOCAL

% \cite{ghaffari2017distributed}: they study upper-bounds for sinkless orientation and graph orientation of $\alpha$-arb graphs in LOCAL. They give $(1+\epsilon)$ approximation.

% \cite{brandt2021randomized}: Give lower-bounds for LLL in the randomized setting. They show that on constant-degree graphs LLL takes $O(\log n)$ LCA queries. Their lower-bound goes via sinkless orientation. They show that {\bf deterministic} coloring a bounded-degree tree with $c \ge 2$ colors, for any fixed constant $c$, takes $\Theta(n)$ VOLUME queries. {\bf \color{red} The last seems quite related to us.}

% \cite{grunau2022landscape}: They prove certain speed-up results for LCLs (locally checkable labelings) and LCAs. Those speed-ups are of the form: if you can solve a problem in $o(\log^\star n)$ complexity, then you can solve it in $O(1)$ as well.

\subparagraph{Orientation and Parnas-Ron paradigm:} 
%\stodo{Explain the approach first. Commonly used to create sublinear algorithms.}

The Parnas-Ron paradigm~\cite{parnas2007approximating} is an important tool for converting distributed algorithms for use in sublinear-time models.
In particular, if there is a $T$-round distributed local algorithm $\cA$, then applying the Parnas-Ron paradigm is equivalent to collecting the $T$-hop neighborhood of a vertex $v$ and using that neighborhood to obtain the output of $\cA$ for $v$, thus getting an LCA with query complexity $O(\D^T)$.

There is a classical peeling algorithm that, given a graph of arboricity at most $\alpha$, finds a $((2 + \eps) \alpha)$-orientation in $O(\log n)$ parallel or LOCAL rounds, for a constant $\eps > 0$. In each step, this algorithm considers all the vertices with degree at most $(2+\eps) \alpha$. All the edges incident to these vertices are oriented outward, and those vertices are then removed from the graph. It is easy to show that this algorithm takes $O(\log n)$ such steps. By following the Parnas-Ron paradigm, in graphs with maximum degree $\Delta$, this peeling algorithm can be simulated with $\Delta^{O(\log n)}$ LCA probes, which yields a trivial upper-bound for any $\Delta > 1$ --- this upper-bound amounts to gathering the entire graph.
If one aims for a more relaxed approximation, e.g., a $\sqrt{\Delta}$-orientation, then the aforementioned peeling algorithm takes $\log_{\sqrt{\Delta}}{n}$ many steps. Nevertheless, even in this case the Parnas-Ron approach yields $\Delta^{\log_{\sqrt{\Delta}}{n}} = n^2$ LCA probe complexity.
Moreover, suppose one aims for any LCA probe complexity that is sublinear in $n$. In that case, the peeling algorithm provides only the guarantee of $\Delta$-approximate orientation, which is trivial to obtain by simply orienting every edge arbitrarily. 


\subparagraph{Orientation and LLL:} Several works study the LCA and the closely related VOLUME complexity of the distributed Lovász local lemma (LLL)~\cite{brandt2016lower,fischer2017sublogarithmic,dorobisz2021local,brandt2021randomized}.
Despite significant progress in understanding the randomized LCA complexity of sinkless orientation and LLL, those techniques do not seem to apply to the problem we study.
In particular, the LLL applies in cases where a random orientation will succeed at most vertices (as is the case with sinkless orientation). However, for the problem of $r$-orientation, a random orientation is very unlikely to be close to correct.


\subparagraph{LCA sparsification:}
One recent development in the LCA model is a graph sparsification technique which is based on considering only a carefully selected subset of the neighbors of a vertex $v$ in order to update the state of $v$. 
This approach has led to new advances for problems such as approximate matching~\cite{ghaffari2019sparsifying,kapralov2020space}, maximal independent set~\cite{ghaffari2019sparsifying,ghaffari2022local}, set cover~\cite{grunau2020improved}, and graph coloring~\cite{chang2019complexity}. However, it is unclear how to apply this technique in the context of $r$-orientation.

\subparagraph{LCA shattering:}
Our approach for bounded-degree forests is reminiscent of the graph-shattering technique, which has been very influential in designing efficient LCA algorithms for a number of problems, including approximate matching~\cite{levi2015local,barenboim2016locality,ghaffari2019sparsifying}, maximal independent set~\cite{rubinfeld2011fast,alon2012space,ghaffari2016improved,barenboim2016locality,ghaffari2019sparsifying}, graph coloring~\cite{barenboim2016locality,chang2019complexity} and LLL algorithms~\cite{alon1991parallel,molloy1998further,fischer2017sublogarithmic,chang2019distributed}. The ideas in this line of work can be traced back to Beck's analysis of the algorithmic LLL~\cite{beck1991algorithmic}. The general idea in these results is to first execute an algorithm that finds only a partial solution, e.g., finds an independent set that is not necessarily maximal. For properly designed algorithms, it can be shown that such an approach ``shatters'' the graph into relatively small connected components of interest, e.g., after removing the found independent set and its neighbors from the graph, each connected component has only $\poly(\Delta)$ vertices. 
These $\poly(\Delta)$ vertices in a single connected component can then be processed with $\poly( \Delta)$ LCA probes with a simple graph traversal.

We remark that our approach departs from this general scheme in the sense that it does not design an algorithm that finds a partial solution first. Instead, it immediately shatters the input tree into more manageable components.

\subparagraph{Other related work:}
Some prior work has also studied the complexity of LCA algorithms in unbounded-degree graphs. For instance, \cite{even2014deterministic} develop an LCA algorithm for $O(\Delta^2 \log \Delta)$-coloring a graph with maximum degree $\Delta = o(\sqrt{n})$. Another work \cite{levi2015local} designs two algorithms for graphs that do not have constant degrees: the first approach is for maximal independent set, which has a quasi-polynomial probe complexity in the maximum degree $\Delta$, while the second approach is for approximating maximum matchings and uses $\poly(\Delta, \log n)$ probes per query. 
Yet another line of work \cite{parter2019spanner, arviv2023spanner} develops an LCA algorithm to construct an $O(k^2)$-spanner with $\Ot(n^{1+1/k})$ edges with probe complexity $n^{2/3-\Omega_k(1)} \poly(\Delta)$.

Several works study the complexity of LLL and related graph problems in LCA, VOLUME, LOCAL, and locally checkable labeling (LCL) models~\cite{goos2015non,brandt2016lower,hefetz2016polynomial,rosenbaum2020seeing,brandt2021randomized,grunau2022landscape,balliu2022distributed}.
We note that our lower-bound applies to the LCA setting, which, as we discuss in \cref{sec:preliminaries}, also applies to the VOLUME model.
The authors of \cite{brandt2021randomized} show that \textit{deterministically} coloring a tree with maximum degree $\poly(c)$ with $c \ge 2$ colors, for any fixed constant $c$, requires $\Theta(n)$ VOLUME probes. 
Another line of work on the hierarchies of VOLUME complexities~\cite{rosenbaum2020seeing} shows that there are graph problems whose randomized VOLUME complexity is $\Theta\rb{n^{c}}$, for any constant $c \in (0, 1)$. 
The celebrated result~\cite{parnas2007approximating} proves that to approximate a vertex cover within a constant factor multiplicative and $\eps n$ additive error, it is necessary to use at least the order of the average degree many probes.
